AMR-Transformer: Enabling Efficient Long-range Interaction for Complex Neural Fluid Simulation

Accurately and efficiently simulating complex fluid dynamics is a challenging task that has traditionally relied on computationally intensive methods. Neural network-based approaches, such as convolutional and graph neural networks, have partially alleviated this burden by enabling efficient local feature extraction. However, they struggle to capture long-range dependencies due to limited receptive fields, and Transformer-based models, while providing global context, incur prohibitive computational costs. To tackle these challenges, we propose AMR-Transformer, an efficient and accurate neural CFD-solving pipeline that integrates a novel adaptive mesh refinement scheme with a Navier-Stokes constraint-aware fast pruning module. This design encourages long-range interactions between simulation cells and facilitates the modeling of global fluid wave patterns, such as turbulence and shockwaves. Experiments show that our approach achieves significant gains in efficiency while preserving critical details, making it suitable for high-resolution physical simulations with long-range dependencies. On CFDBench, PDEBench and a new shockwave dataset, our pipeline demonstrates up to an order-of-magnitude improvement in accuracy over baseline models. Additionally, compared to ViT, our approach achieves a reduction in FLOPs of up to 60 times.

==> sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> texts/method_backup.tex <==
\section{Method}
\label{sec:method}
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=0.99\textwidth]{AMRT_pipeline/main_pipeline_test_03.png}
    \vspace{-1em}
    \captionof{figure}{\textbf{AMR-Transformer Pipeline:} Demonstrated in the shockwave case. Our AMR-Transformer pipeline combines Adaptive Mesh Refinement (AMR) as a tokenizer with a Transformer neural solver to capture complex fluid dynamics. By adaptively refining regions of interest, AMR reduces computational costs while preserving essential flow details, enabling the Transformer to efficiently model interactions across multiple scales. This approach achieves a balance between accuracy and computational efficiency.}
    \label{fig:pipeline}
\end{figure*}

Traditional methods, such as CNN-based approaches, are unable to model long-range interactions effectively, while using Transformers with self-attention for direct interaction modeling is too slow when handling high-resolution data. In order to alleviate the problem, We present the AMR-Transformer Pipeline (Section~\ref{sec:pipeline}), outlining the transformation of structured grids into a multi-scale representation using a hierarchical AMR Tokenizer (Section~\ref{sec:tokenizer}). The Encoder-only Transformer Neural Solver (Section~\ref{sec:neuralsolver}) then applies self-attention across patches with positional encoding, enabling the model to learn dependencies across scales. Finally, we detail our model training and testing setup (Section~\ref{sec:train}), discussing loss function, label tokenization, and pruning criteria for precise multi-scale simulation.

\subsection{AMR-Transformer Pipeline}
\label{sec:pipeline}
    We propose a novel pipeline, the AMR-Transformer (Figure \ref{fig:pipeline}), which combines Adaptive Mesh Refinement (AMR) as a tokenizer with a Transformer-based neural solver. Grid-based AMR processing transforms the feature domain from the structured grid \(\mathbb{R}^{H \times W \times p}\), where each region has \(p\)-dimensional features, to a patch representation \(\mathbb{R}^{N \times K \times p}\). Here, \(N\) denotes the number of patches, each patch contains \(K\) regions. For adaptive refinement, we employ a multi-way tree structure, and the Nested AMR produces overlapping patches of varying sizes. This transformation allows the Transformer to take patches directly as inputs, where the self-attention mechanism models interactions across multiple scales within the adaptive resolution provided by AMR.
    
\subsection{AMR Tokenizer}
\label{sec:tokenizer}
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.48 \textwidth]{AMRT_pipeline/AMR_tokenizer_01.png}
%     \caption{\textbf{Condition Evaluation:} Demonstrated in the cylinder flow problem, the AMR tokenizer adaptively refines regions based on Kelvin-Helmholtz Instability and Velocity Gradient conditions. Each level calculates refinement regions for both conditions, taking their union to determine areas for further subdivision in the next level.}
%     \label{fig:tokenizer}
% \end{figure}

    The AMR Tokenizer employs a nested multi-way tree adaptive mesh refinement (AMR) strategy to capture multi-scale features in fluid dynamics data (Figure \ref{fig:amr_problems}). For simplicity, we illustrate the method in 2D using a quadtree structure; this approach can easily generalizes to 3D with an octree or multi-way tree. In this framework, the tokenizer partitions the input domain based on specific physical criteria, transforming the structured grid into a set of patches, where each patch contains \( k \times k \) regions. The parameter \( k \) determines the number of subdivisions per dimension and directly influences the resolution of the patches. This hierarchical representation preserves essential feature information at different levels, facilitating multi-scale analysis and reconstruction within the Transformer pipeline.
    The pipeline is shown in Algorithm~\ref{alg:amr_tokenizer}.
    
    \paragraph{Parallel Processing Implementation}
        To enhance computational efficiency, we process all regions at a given depth level in parallel before proceeding to the next level. This approach significantly speeding up the pruning process. The key steps of the AMR tokenizer are as follows:
        
        \begin{enumerate}
            \item \textbf{Initialization}: Define the entire input domain as a singular region to initiate the pruning process.
        
            \item \textbf{N-S Constraint-Aware Pruning Module}: The Navier-Stokes constraint-aware fast pruning module evaluates the pruning conditions for all regions concurrently at the current depth level, utilizing relevant physical quantities such as velocity gradients, vorticity, momentum, and the criteria for Kelvin-Helmholtz instability.

            \item \textbf{Decision Making}: Based on the results of the condition evaluation, categorize each region as follows:
            \begin{itemize}
                \item \textbf{Subdivide and Retain}: If a region meets the pruning criteria, subdivide it into \(k \times k\) smaller regions and retain it for further processing.
                
                \item \textbf{Retain without Subdivision}: If a region meets the criteria for storage, retain it without further subdivision.
                
                \item \textbf{Disregard}: Regions that do not meet the refinement or storage criteria are completely disregarded, meaning they are neither stored nor subdivided.
                
                \item \textbf{Subdivide but Disregard}: Regions that require subdivision but do not meet the criteria for storage are subdivided for potential future processing without retaining their data.
            \end{itemize}
            
            \item \textbf{Patch Formation}:
            \begin{itemize}
                \item \textbf{Feature Aggregation for Regions}: For each region designated for storage, compute the feature vector \(f_C\) for each region \(C\) by averaging the values of data points \(\{ x_i \}\) contained within \(C\):
                \[
                f_C = \frac{1}{|C|} \sum_{x_i \in C} x_i
                \]
                
                \item \textbf{Patch Assembly}: Construct a patch representation by combining the feature vectors from the \(k \times k\) regions into a single collection:
                \[
                \text{Patch} = \{ f_{C_{1,1}}, f_{C_{1,2}}, \ldots, f_{C_{k,k}} \}
                \]
                
                \item \textbf{Positional Embedding}: Enhance the patch representation by appending positional information, which includes the depth \(d\) and the mean coordinates \((\bar{x}, \bar{y})\) of the regions within the patch. The comprehensive representation of the patch \( \text{Patch}_C \) can thus be expressed as:
                \[
                \text{Patch}_C = [f_C, d, \bar{x}, \bar{y}]
                \]
            \end{itemize}
            
            \item \textbf{Iteration}: Collect all newly formed regions from the subdivision process and repeat the evaluation and decision-making steps in parallel at the subsequent depth level.
            
            \item \textbf{Termination}: Conclude the process when all regions have been either subdivided to the minimum allowable size or transformed into patches, ensuring that no regions remain for further processing.
        \end{enumerate}
    
    \paragraph{N-S Constraint-Aware Pruning Module}
       The module applies pruning based on specific physical properties that are crucial for capturing the complex dynamics of fluid flow. By concentrating computational resources in these regions, we ensure higher resolution where it matters most, thereby enhancing simulation accuracy. Each criterion is designed to capture unique aspects of fluid motion, ranging from localized rapid changes to instability-induced turbulence. These conditions and their theoretical foundations are described as follows:
                
        \begin{itemize}
            \item \textbf{Velocity Gradient:} The velocity gradient detects sharp changes in fluid speed, which often appear at boundaries, shock fronts, or regions where fine-scale features emerge. For example, in shockwave and dam break scenarios, sudden velocity shifts create high gradients that signify discontinuities or fronts. We compute the gradient magnitude \( G \) as:
            \[
            G = \sqrt{\left| \nabla u \right|^2 + \left| \nabla v \right|^2},
            \]
            where \( \nabla u \) and \( \nabla v \) represent spatial velocity changes. Capturing these shifts is critical for delineating features like shock fronts and complex flow boundaries, enhancing the model's ability to track rapid transitions and flow separations.
        
            \item \textbf{Vorticity:} Vorticity \( \omega \), defined as 
            \[
            \omega = \frac{\partial v}{\partial x} - \frac{\partial u}{\partial y},
            \]
            measures local fluid rotation, indicating swirling flows like eddies or turbulence. High vorticity often characterizes regions where rotational motion drives turbulent mixing and energy dissipation, as seen in cavity flows or behind cylindrical obstacles. Identifying these zones ensures that vortex structures are resolved, supporting a detailed representation of rotational flow behavior crucial for understanding energy transfer within the fluid.
        
            \item \textbf{Momentum:} This condition identifies regions with significant flow momentum, which heavily influence the overall dynamics. High-momentum areas are crucial in problems where flow jets or moving currents, like those in tube or dam flows, dictate the system’s behavior. The momentum \( P \) of a region, calculated from the total components \( P_x \) and \( P_y \):
            \[
            P = \sqrt{P_x^2 + P_y^2}, \quad P_x = \int u \, dA, \quad P_y = \int v \, dA.
            \]
            Capturing momentum-heavy regions helps the model simulate critical flow-driving forces accurately, which impacts downstream behavior and the interaction of moving fronts with boundaries.
        
            \item \textbf{Kelvin-Helmholtz Instability:} This criterion detects shear-driven instabilities, like the Kelvin-Helmholtz instability, which forms at fluid interfaces with significant velocity differentials. Such shear instabilities are common in atmospheric flows and can be relevant in tube and dam break scenarios, where layers of moving fluid interact. The shear strength \( S \), defined as:
            \[
            S = \left| \frac{\partial u}{\partial y} - \frac{\partial v}{\partial x} \right|,
            \]
            helps pinpoint areas prone to instability, allowing the model to depict the emergence of wave patterns and subsequent turbulence. This capability is essential for resolving the fine-scale interfacial interactions that contribute to mixing and layer formation.
        \end{itemize}

        % More details on the specific threshold settings and condition evaluation methods can be found in Appendix \ref{sec:threshold_and_condition_appendix}.

\begin{algorithm}[htbp]
    \caption{AMR Tokenizer Pipeline}
    \label{alg:amr_tokenizer}
    \begin{algorithmic}[1]
        \State \textbf{Input:} Structured grid $\mathbb{R}^{H \times W \times p}$ with $p$-dimensional features
        \State \textbf{Output:} Set of patches $\mathbb{R}^{N \times K \times p}$

        \State Initialize the entire input domain as a single region
        \State Initialize a queue with the region at depth $d = 0$
        
        \While{queue is not empty}
            \State Extract all regions at the current depth level $d$
            \State Evaluate pruning conditions for each region based on physical criteria:
            \For{each region $R$ in the current depth level}
                \If{$R$ meets pruning conditions}
                    \State Subdivide $R$ into $k \times k$ smaller regions
                    \State Add the subdivided regions to the queue for depth $d + 1$
                \EndIf
                \If{$R$ meets storage conditions}
                    \State Generate patches for region $R$
                \EndIf
            \EndFor
            \State Increment depth level $d \gets d + 1$
        \EndWhile
        
        \State \textbf{Return:} Generated patches
    \end{algorithmic}
\end{algorithm}

    
\subsection{Transformer Neural Solver}
\label{sec:neuralsolver}
% 可以删减
    After processing the input domain through the AMR Tokenizer, we generate a structured set of patches that are sorted by position and encoded with 3D sinusoidal positional information, incorporating two spatial coordinates \(x\), \(y\), and one depth level \(d\). This positional encoding transforms each patch into a token, providing spatial context for the Encoder-only Transformer neural solver to model multi-scale interactions across the tokens.
    
    Given a sequence of \(N\) sorted tokens, each represented by a feature vector \(f_i\), the self-attention mechanism computes multi-head attention with query \(Q\), key \(K\), and value \(V\) matrices derived from the encoded tokens:
    \[
    Q = f_i W^Q, \quad K = f_i W^K, \quad V = f_i W^V,
    \] 
    where \( W^Q \), \( W^K \), and \( W^V \) are learnable projection matrices. The self-attention score \( \text{Attention}(Q, K, V) \) is computed as:
    \[
    \text{Attention}(Q, K, V) = \text{softmax}\left( \frac{Q K^\top}{\sqrt{d_k}} \right) V,
    \]
    where \( d_k \) is the dimensionality of the key vectors. 
    % This formulation enables the Transformer to capture long-range dependencies across the multi-scale tokens efficiently, leveraging both local and global information to represent the complex interactions in fluid dynamics simulations.
    
\subsection{Model Training and Testing}
\label{sec:train}
    During training, we randomly generate the hyperparameters for the subdivision criteria, allowing the AMR pruning parameters to be manually adjusted after model training. This flexibility enables further optimization of the tradeoff between accuracy and computational efficiency.
    Following \cite{cfdbench}, we use the normalized mean squared error (NMSE) as the loss function, which normalizes the error across different scales, making it suitable for evaluating high-precision fluid simulations.
    
    The training labels are processed through the AMR Tokenizer, resulting in tokenized labels that match the multi-scale representation of the model’s output. During testing, however, we map the model’s output back onto the original regular grid, enabling direct comparison with the ground truth label on the original domain.
    
    To improve the fidelity of the pruning conditions, we use the velocity fields from both the current and previous time steps, applying forward Euler integration to estimate a virtual velocity field for the next time step. The current and virtual velocity fields are then used as input for the pruning criteria, with their results combined to determine the final set of pruning regions.
    
    % , specifically designed to capture long-range dependencies in 2D CFD problems. 
    % Compared to traditional convolutional neural networks (CNNs), implicit neural representation (INR) models such as DeepONet, Neural Fourier Machines (NFM), and neural operators (NO) like Fourier Neural Operator (FNO), the Transformer architecture effectively leverages patches as tokens. Each patch token, represented as \(\mathbb{R}^{k \times D}\), encapsulates local fluid dynamics at an adaptively refined resolution, which is tailored to the complexity of the region. The self-attention mechanism in the Transformer enables efficient and accurate modeling of long-range dependencies across the simulation domain, facilitating multiscale information processing without incurring prohibitive computational costs.
    


% 符号表
